Complete ZX-calculi for the stabiliser fragment in odd prime dimensions

We introduce a family of ZX-calculi which axiomatise the stabiliser fragment of quantum theory in odd prime dimensions. These calculi recover many of the nice features of the qubit ZX-calculus which were lost in previous proposals for higher-dimensional systems. We then prove that these calculi are complete, i.e. provide a set of rewrite rules which can be used to prove any equality of stabiliser quantum operations. Adding a discard construction, we obtain a calculus complete for mixed state stabiliser quantum mechanics in odd prime dimensions, and this furthermore gives a complete axiomatisation for the related diagrammatic language for affine co-isotropic relations.

==> app_proofs.tex <==
\subsection{Proof of soundness}
\label{app:proofs:soundness}



\begin{proof}[Proof of theorem~\ref{thm:soundness}]
  We prove that each of the equations in figure~\ref{fig:axioms} is sound, and
  this extends to the entire equational theory by functoriality of
  \(\interp{-}\).

  Firstly, straightforward calculation shows that:
  \begin{equation}
    \label{eq:scalars}
    \interp{\tikzfig{figures/equations/soundness/sqroot_d_inv}} = \frac{1}{\sqrt{p}}
    \qc
    \interp{\tikzfig{figures/equations/soundness/sqroot_d}} = \sqrt{p} \omega^{-2^{-1}xz},
    % \qc
    % \interp{\tikzfig{figures/equations/soundness/d}} = p,
    \qand
    \interp{\tikzfig{figures/equations/soundness/d_phase}} = \sum_{m\in\Z_p} \omega^{2^{-1}(xm + ym^2)}.
  \end{equation}

  \textsc{(Scalar)} follows immediately from equation~\eqref{eq:scalars}.

  (H) For any \(m,n \in \Z_p\),
  \begin{align}
    \interp{\tikzfig{figures/equations/soundness/H_RHS}}
    % &= \frac{1}{\sqrt p} \sum_{x,y,z\in\Z_p} \omega^{2^{-1}x^2} \omega^{2^{-1}y^2} \omega^{2^{-1}z^2} \ip{x:X}{y:Z} \ip{y:Z}{-z:X} \dyad{-x:X}{z:X} \\
    &= \frac{1}{\sqrt p} \sum_{x,y,z\in\Z_p} \omega^{2^{-1}x^2} \omega^{2^{-1}y^2} \omega^{2^{-1}z^2} \omega^{-xy} \omega^{-yz} \dyad{-x:X}{z:X} \\
    &= \frac{1}{\sqrt p} \sum_{x,y,z\in\Z_p} \omega^{2^{-1}x^2} \omega^{2^{-1}y^2} \omega^{2^{-1}z^2} \omega^{-xy} \omega^{-yz} \dyad{-x:X}{z:X} \\
    &= \frac{1}{\sqrt p} \sum_{x,y,z\in\Z_p} \omega^{2^{-1}x^2} \omega^{2^{-1}y^2} \omega^{2^{-1}z^2} \omega^{-xy} \omega^{-yz} \dyad{-x:X}{z:X} \\
    &= \frac{1}{\sqrt p} \sum_{x,y,z\in\Z_p} \omega^{2^{-1}x^2} \omega^{2^{-1}y^2} \omega^{2^{-1}z^2} \omega^{-xy} \omega^{-yz} \omega^{xz} \omega^{-xz} \dyad{-x:X}{z:X} \\
    &= \frac{1}{\sqrt p} \sum_{x,y,z\in\Z_p} \omega^{2^{-1}(x^2 + y^2 + z^2 - 2xy - 2yz + 2xz)} \omega^{-xz} \dyad{-x:X}{z:X} \\
    &= \frac{1}{\sqrt p} \sum_{x,z\in\Z_p} \left( \sum_{y\in\Z_p} \omega^{2^{-1}(x-y+z)^2} \right) \omega^{-xz} \dyad{-x:X}{z:X} \\
    &= \left( \sum_{y\in\Z_p} \omega^{2^{-1}y^2} \right) \frac{1}{\sqrt{p}} \sum_{x,z\in\Z_p} \omega^{xz} \dyad{x:X}{z:X} \\
    &= \left( \sum_{y\in\Z_p} \omega^{2^{-1}y^2} \right) \cdot \sum_{x\in\Z_p} \dyad{x:X}{x:Z} \\
    &= \interp{\tikzfig{figures/equations/soundness/H_LHS}},
  \end{align}
  where we have used the change of variables \(y \mapsto y + x + z\) which preserves
  the sum over \(y\in\Z_p\) for any \(x,z \in \Z_p\).

  \textsc{(Mult)} For any \(z \in \Z_p^*\),
  \begin{align}
    \interp{\tikzfig{figures/equations/soundness/Mult_RHS}}
    % &= p \sum_{a,b,c,d\in\Z_p} \omega^{2^{-1}z^{-1}a^2} \omega^{2^{-1}zb^2} \omega^{2^{-1}z^{-1}c^2} \ip{a:Z}{-b:X} \ip{b:X}{c:Z} \ip{c:Z}{d:Z} \dyad{a:Z}{d:X} \\
    &= \sum_{a,b,c,d\in\Z_p} \omega^{2^{-1}z^{-1}a^2} \omega^{2^{-1}zb^2} \omega^{2^{-1}z^{-1}c^2} \omega^{-ab} \omega^{-bc} \delta_{c,d} \dyad{a:Z}{d:X} \\
    &= \sum_{a,b,c\in\Z_p} \omega^{2^{-1}z^{-1}a^2} \omega^{2^{-1}zb^2} \omega^{2^{-1}z^{-1}c^2} \omega^{-ab} \omega^{-bc} \dyad{a:Z}{c:X} \\
    &= \sum_{a,b,c\in\Z_p} \omega^{2^{-1}z^{-1}(a-zb+c)^2} \omega^{-z^{-1}ac} \dyad{a:Z}{c:X} \\
    &= \left( \sum_{b\in\Z_p} \omega^{2^{-1}z^{-1}b^2} \right) \sum_{a,c\in\Z_p} \omega^{-z^{-1}ac} \dyad{a:Z}{c:X} \\
    &= \left( \sum_{b\in\Z_p} \omega^{2^{-1}z^{-1}b^2} \right) \sqrt{p} \sum_{a\in\Z_p} \dyad{a:Z}{z^{-1}a:Z} \\
    &= \left( \sum_{b\in\Z_p} \omega^{2^{-1}z^{-1}b^2} \right) \sqrt{p} \sum_{a\in\Z_p} \dyad{za:Z}{a:Z} \\
    &= \left( \sum_{b\in\Z_p} \omega^{2^{-1}z^{-1}b^2} \right) \sum_{a,c\in\Z_p} \omega^{-zac} \dyad{c:X}{a:Z} \\
    &= \left( \sum_{b\in\Z_p} \omega^{2^{-1}z^{-1}b^2} \right) \sqrt{p^z} \sum_{a,c\in\Z_p} \dyad{c:X}{c:X}^{\otimes z} \ket{a:Z}^{\otimes z}\bra{a:Z} \\
    &= \interp{\tikzfig{figures/equations/soundness/Mult_LHS}}.
  \end{align}
\end{proof}
